Experimental Analysis of Tip Vortex Cavitation Mitigation By Controlled Surface Roughness

This study presents results of experiments where roughness applications are evaluated in delaying the tip vortex cavitation inception of an elliptical foil. High-speed video recordings and Laser Doppler Velocimetry (LDV) measurements are employed to provide further details on the cavitation behaviour and tip vortex flow properties in different roughness pattern configurations. The angular momentum measurements of the vortex core region at one chord length downstream of the tip indicate that roughness leads to a lower angular momentum compared to the smooth foil condition while the vortex core radius remains similar in the smooth and roughened conditions. The observations show that the cavitation number for tip vortex cavitation inception is reduced by 33 % in the optimized roughness pattern compared to the smooth foil condition where the drag force increase is observed to be around 2 %. During the tests, no obvious differences in the cavitation inception properties of uniform and non-uniform roughness distributions are observed. However, the drag force is found to be higher with a non-uniform roughness distribution.

==> texFiles/GraphicalAbstract.tex <==
\section{Graphical abstract}

\begin{figure}[h!]
		\centering               
		\begin{subfigure}[b]{0.4\textwidth}
			  \begin{tikzpicture}
			  \node [anchor=south west,inner sep=0](mesh)at(0,0){
			  \includegraphics[width=\textwidth]{Figure/Picture1.png} 
								};
				\fill[fill=yellow] (1.5,3.0) node [fill=red!5,draw,double,rounded corners] {\large Sparse roughness};		
			  \end{tikzpicture}	 				  
        \end{subfigure} 
        \quad
		\begin{subfigure}[b]{0.4\textwidth}
			  \begin{tikzpicture}
			  \node [anchor=south west,inner sep=0](mesh)at(0,0){
			  \includegraphics[width=\textwidth]{Figure/Picture2.png} 
								};
				\fill[fill=yellow] (0.75,3.0) node [fill=red!5,draw,double,rounded corners] {\large Smooth};
			  \end{tikzpicture}	  				  
		\end{subfigure} 
		\captionsetup{labelformat=empty}
\end{figure}
\setcounter{figure}{0}





==> texFiles/Resuslts/newMaterials.tex <==
\noindent
For the smooth 
 
\begin{figure} [h!]	
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
        		  \includegraphics[width=\textwidth]{Figure/ReynoldsImpact/sigma26Va28.png}
				  \caption{Re=$8.55 \times 10^5$}
                  \label{fig::SmoothSigma12MaxMin}
        \end{subfigure}
        \begin{subfigure}[b]{0.45\textwidth}
				  \includegraphics[width=\textwidth]{Figure/ReynoldsImpact/sigma26Va40.png}
				  \caption{Re=$1.204 \times 10^6$}
                  \label{fig::tipRoughSigma12MaxMin}
        \end{subfigure}  
		\caption{Impact of Reynolds number on TVC, smooth foil, zoomed view of the suction side tip, $\sigma=2.6$, $\alpha$= 9$^\circ$.}          
		 \label{fig::SmoothRoughSigma12MaxMin}                   	
\end{figure}


\begin{comment}
5
\end{comment}


